Nonlinear consensus protocols with applications to quantized systems

This paper studies multi-agent systems with nonlinear consensus protocols, i.e., only nonlinear measurements of the states are available to agents. The solutions of these systems are understood in Filippov sense since the possible discontinuity of the nonlinear controllers. Under the condition that the nonlinear functions are monotonic increasing without any continuous constraints, asymptotic stability is derived for systems defines on both directed and undirected graphs. The results can be applied to quantized consensus which extend some existing results from undirected graphs to directed ones.

==> user_newcommands.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% RANDOM
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\addtolength{\headheight}{14pt}
%\newcommand{\xend}{\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill \quad\hbox{\ensuremath{\lozenge}}} % end environment (e.g. example)
\newcommand{\addcontentslineX}[3]{\phantomsection \addcontentsline{#1}{#2}{#3}} % this command guarantees correct hyperlinks in the pdf to those sections that are not numbered (e.g. acknowledgements, summary, etc.)
\newcommand{\todo}[1] {\textcolor{red}{{#1}}}
\def\str{\color{red}} %STart Red
\def\stb{\color{black}} %STart Black
\newcommand{\publ}{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% COLOR
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\definecolor{cof}{RGB}{219,144,71}
\definecolor{pur}{RGB}{186,146,162}
\definecolor{greeo}{RGB}{91,173,69}
\definecolor{greet}{RGB}{52,111,72}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% cross text
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[normalem]{ulem} % either use this (simple) or
\usepackage{soul}
\usepackage{cancel}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% BIBLIOGRAPHY
% Commands for full citations (NoHyper is used to  solve conflict with hyperref)
% \fullciteInclude includes full citation into bibliography
% \fullciteExclude excludes full citation from bibliography
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\fullcite}[1]{\begin{NoHyper} \bibentry{#1} \end{NoHyper}}
%\DeclareBibliographyCategory{fullcited}
%\newcommand{\mybibexclude}[1]{\addtocategory{fullcited}{#1}}
%\newcommand{\fullciteInclude}[1]{\begin{NoHyper} \fullcite{#1} \end{NoHyper}}
%\newcommand{\fullciteExclude}[1]{\begin{NoHyper} \fullcite{#1}\mybibexclude{#1} \end{NoHyper}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% FIGURES
% Commands for including figures/plots in a standard sizing
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\includegraphicsfig}[1] {\includegraphics[width=80mm,height=60mm,keepaspectratio]{#1}} % Include figure
\newcommand{\includegraphicsplot}[1] {\includegraphics[width=95mm]{#1}} % Include MATLAB plot
%\usepackage{pgfplots}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% MATH
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bal}[1] {\ensuremath{\left(\begin{array}{#1}}}
\newcommand{\ear} {\ensuremath{\end{array}\right)}}
\newcommand{\pd}[2] {\ensuremath{\frac{\partial #1}{\partial #2}}}
%\newcommand{\col}[1] {\ensuremath{\left(#1\right)^T}} %column vector in math mode
%\newcommand{\diag}[1] {\ensuremath{\mathrm{diag}\left(#1\right)}} %diagonal matrix in math mode
%\newcommand{\bdiag}[1] {\ensuremath{\mathrm{block.diag}\left(#1\right)}} %diagonal matrix in math mode
\newcommand{\col}[1] {\ensuremath{#1^T}} %column vector in math mode
%\newcommand{\diag}[1] {\ensuremath{\mathrm{diag}(#1)}} %diagonal matrix in math mode
\newcommand{\bdiag}[1] {\ensuremath{\mathrm{block.diag}(#1)}} %diagonal matrix in math mode
\newcommand{\bals}[1] {\ensuremath{\left[\begin{array}{#1}}} % Begin Array Left Square
\newcommand{\ears} {\ensuremath{\end{array} \right] }} % End Array Right Square
\newcommand{\one}[1] {\ensuremath{\mathds{1}_{#1} }} % Vector of ones
\newcommand{\co} {\ensuremath{\mathrm{co}}} % Convex hull



\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\spa}{span}
\DeclareMathOperator{\sat}{sat}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\inte}{int}
\DeclareMathOperator{\clo}{cl}
\DeclareMathOperator{\rint}{rint}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\cone}{cone}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\graph}{graph}
\DeclareMathOperator{\dis}{dis}
\DeclareMathOperator{\Real}{Re}
\DeclareMathOperator{\Imag}{Im}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\arctantwo}{arctan2}
\DeclareMathOperator{\SAT}{SAT}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\diag}{diag}


\newcommand{\funcRdR}{\ensuremath{{f}}}
\newcommand{\funcRdRd}{\ensuremath{{X}}}

%\DeclareMathOperator{\ones}{{\ensuremath\mathds{1}_n}}

\newcommand{\signf}[1]{\ensuremath{\sign \left( #1 \right)}} % sign function
\DeclareMathOperator*{\bigtimes}{\raisebox{-0.3ex}{\text{\Large$\times$}}}
\newcommand{\inproduct}[1]{\ensuremath{\left\langle #1 \right\rangle}}

\let\leq\leqslant
\let\geq\geqslant
\let\emptyset\varnothing

\newcommand{\calA}{\ensuremath{\mathcal{A}}}
\newcommand{\calB}{\ensuremath{\mathcal{B}}}
\newcommand{\calC}{\ensuremath{\mathcal{C}}}
\newcommand{\calD}{\ensuremath{\mathcal{D}}}
\newcommand{\calE}{\ensuremath{\mathcal{E}}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\calG}{\ensuremath{\mathcal{G}}}
\newcommand{\calH}{\ensuremath{\mathcal{H}}}
\newcommand{\calI}{\ensuremath{\mathcal{I}}}
\newcommand{\calJ}{\ensuremath{\mathcal{J}}}
\newcommand{\calK}{\ensuremath{\mathcal{K}}}
\newcommand{\calL}{\ensuremath{\mathcal{L}}}
\newcommand{\calM}{\ensuremath{\mathcal{M}}}
\newcommand{\calN}{\ensuremath{\mathcal{N}}}
\newcommand{\calO}{\ensuremath{\mathcal{O}}}
\newcommand{\calP}{\ensuremath{\mathcal{P}}}
\newcommand{\calQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\calR}{\ensuremath{\mathcal{R}}}
\newcommand{\calS}{\ensuremath{\mathcal{S}}}
\newcommand{\calT}{\ensuremath{\mathcal{T}}}
\newcommand{\calU}{\ensuremath{\mathcal{U}}}
\newcommand{\calV}{\ensuremath{\mathcal{V}}}
\newcommand{\calW}{\ensuremath{\mathcal{W}}}
\newcommand{\calX}{\ensuremath{\mathcal{X}}}
\newcommand{\calY}{\ensuremath{\mathcal{Y}}}
\newcommand{\calZ}{\ensuremath{\mathcal{Z}}}

\newcommand{\frakm}{\ensuremath{\mathfrak{m}}} % the lebesgue measure



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ENVIRONMENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bmat}{\begin{matrix}}
\newcommand{\emat}{\end{matrix}}
\newcommand{\bbm}{\begin{bmatrix}}
\newcommand{\ebm}{\end{bmatrix}}
\newcommand{\bpm}{\begin{pmatrix}}
\newcommand{\epm}{\end{pmatrix}}
\newcommand{\bse}{\begin{subequations}}
\newcommand{\ese}{\end{subequations}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
%\newcommand{\beq*}{\begin{equation*}}
%\newcommand{\eeq*}{\end{equation*}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\beni}{\renewcommand{\labelenumi}{\roman{enumi}.}
\renewcommand{\theenumi}{\roman{enumi}}\begin{enumerate}}
\newcommand{\eeni}{\end{enumerate}\renewcommand{\labelenumi}{\arabic{enumi}.}
\renewcommand{\theenumi}{\arabic{enumi}}}
\newcommand{\bena}{\renewcommand{\labelenumi}{\alpha{enumi}.}
\renewcommand{\theenumi}{\alpha{enumi}}\begin{enumerate}}
\newcommand{\eena}{\end{enumerate}\renewcommand{\labelenumi}{\arabic{enumi}.}
\renewcommand{\theenumi}{\arabic{enumi}}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  SHORTHAND MATH
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ones}{\ensuremath{1\!\!1}}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\half}{\ensuremath{\frac{1}{2}}}
\newcommand{\inv}{\ensuremath{^{-1}}}
\newcommand{\pset}[1]{\ensuremath{\{#1\}}}
\newcommand{\nset}[1]{\ensuremath{\{1,2,\ldots,#1\}}}
\newcommand{\setzero}{\ensuremath{\pset{0}}}
\newcommand{\lexleq}{\ensuremath{\preccurlyeq}}
\newcommand{\lexgeq}{\ensuremath{\succcurlyeq}}
\newcommand{\set}[2]{\ensuremath{\{#1\mid #2\}}}
\newcommand{\res}[2]{\ensuremath{#1|_{#2}}}
\newcommand{\abs}[1]{\ensuremath{| #1 |}}
\newcommand{\norm}[1]{\ensuremath{\| #1 \|}}
\newcommand{\inn}[2]{\ensuremath{\langle #1 , #2 \rangle}}
\newcommand{\polar}[1]{\ensuremath{{#1}^\circ}}
\newcommand{\dual}[1]{\ensuremath{{#1}^*}}
\newcommand{\barrier}[1]{\ensuremath{{#1}^{\mathrm{b}}}}
\newcommand{\rec}[1]{\ensuremath{{#1}^{\infty}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  SETS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\R}{\ensuremath{\mathbb R}}
\newcommand{\C}{\ensuremath{\mathbb C}}
\newcommand{\N}{\ensuremath{\mathbb N}}
\newcommand{\Z}{\ensuremath{\mathbb Z}}
\newcommand{\Lone}{\ensuremath{L_1}}
\newcommand{\Loneloc}{\ensuremath{L_{1,\mathrm{loc}}}}
\newcommand{\Ltwo}{\ensuremath{L_2}}
\newcommand{\Ltwoloc}{\ensuremath{L_{2,\mathrm{loc}}}}
\newcommand{\Linf}{\ensuremath{L_\infty}}
\newcommand{\Linfloc}{\ensuremath{L_{\infty,\mathrm{loc}}}}
\newcommand{\Cinf}{\ensuremath{C^\infty}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  EMPTY CHAPTER PAGES BEFORE EACH CHAPTER
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcounter{foochapter} % counter for chapter frontpage

\newcommand{\addchapterfront}{
\setcounter{foochapter}{\the\value{chapter}}
\stepcounter{foochapter}
\cleardoublepage
\thispagestyle{empty}
\vspace*{40mm}
\begin{flushright}
\fontfamily{ugm}\textrm{\huge Chapter~}
\color{RoyalRed}\fontfamily{ugm}\fontsize{70}{70}\selectfont\the\value{foochapter} \\
\vspace{2mm}
\color{black}\hrule
\vspace{2mm}
\includegraphics[height = 20.3mm]{./front/bw_logo_rug}
%{ \Large \nameref*{chap:\the\value{foochapter}} }
\end{flushright}
\renewcommand{\thepage}{[\arabic{page}]}
\cleardoublepage
\addtocounter{page}{-2}
\renewcommand{\thepage}{\arabic{page}}
}

\newcommand{\addappendixfront}{
\cleardoublepage
\thispagestyle{empty}
\vspace*{40mm}
\begin{flushright}
\textbf{\huge Appendix }\\
\vspace{2mm}
\hrule
\end{flushright}
\renewcommand{\thepage}{[\arabic{page}]}
\cleardoublepage
\addtocounter{page}{-2}
\renewcommand{\thepage}{\arabic{page}}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FONTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\renewcommand{\sfdefault}{mdugm}
\renewcommand{\sfdefault}{ugm}




%\newboolean{garamond}
%\DeclareOption{garamond}{\setboolean{garamond}{true}}
%
%\ifthenelse{\boolean{garamond}}
%{%
%  \ifpdf
%   \RequirePackage[T1]{fontenc} 
%   \RequirePackage[urw-garamond]{mathdesign}
%   \RequirePackage[scaled]{berasans} 
%   \RequirePackage{inconsolata} % tt
%   \linespread{1.0609}
%  \fi}%
%{}
